On the inequalities of Babu\v{s}ka-Aziz, Friedrichs and Horgan-Payne

The equivalence between the inequalities of Babu\v{s}ka-Aziz and Friedrichs for sufficiently smooth bounded domains in the plane has been shown by Horgan and Payne 30 years ago. We prove that this equivalence, and the equality between the associated constants, is true without any regularity condition on the domain. For the Horgan-Payne inequality, which is an upper bound of the Friedrichs constant for plane star-shaped domains in terms of a geometric quantity known as the Horgan-Payne angle, we show that it is true for some classes of domains, but not for all bounded star-shaped domains. We prove a weaker inequality that is true in all cases.

==> filelogspic2-58.tex <==
   -1.0000   -0.0000
   -0.9602   -0.0151
   -0.9217   -0.0290
   -0.8845   -0.0417
   -0.8487   -0.0534
   -0.8141   -0.0641
   -0.7807   -0.0738
   -0.7485   -0.0826
   -0.7174   -0.0906
   -0.6875   -0.0978
   -0.6586   -0.1043
   -0.6308   -0.1101
   -0.6040   -0.1152
   -0.5782   -0.1197
   -0.5534   -0.1237
   -0.5294   -0.1271
   -0.5064   -0.1300
   -0.4843   -0.1325
   -0.4630   -0.1345
   -0.4425   -0.1361
   -0.4229   -0.1374
   -0.4039   -0.1383
   -0.3858   -0.1389
   -0.3683   -0.1392
   -0.3515   -0.1392
   -0.3354   -0.1389
   -0.3200   -0.1385
   -0.3051   -0.1378
   -0.2909   -0.1369
   -0.2773   -0.1358
   -0.2642   -0.1346
   -0.2516   -0.1332
   -0.2396   -0.1317
   -0.2280   -0.1301
   -0.2170   -0.1283
   -0.2064   -0.1265
   -0.1963   -0.1246
   -0.1866   -0.1226
   -0.1773   -0.1205
   -0.1684   -0.1184
   -0.1599   -0.1162
   -0.1518   -0.1140
   -0.1440   -0.1117
   -0.1366   -0.1095
   -0.1295   -0.1072
   -0.1228   -0.1048
   -0.1163   -0.1025
   -0.1101   -0.1002
   -0.1042   -0.0979
   -0.0986   -0.0955
   -0.0932   -0.0932
   -0.0881   -0.0909
   -0.0832   -0.0886
   -0.0786   -0.0863
   -0.0741   -0.0841
   -0.0699   -0.0819
   -0.0659   -0.0796
   -0.0621   -0.0775
   -0.0584   -0.0753
   -0.0550   -0.0732
   -0.0517   -0.0711
   -0.0485   -0.0691
   -0.0456   -0.0670
   -0.0427   -0.0651
   -0.0400   -0.0631
   -0.0375   -0.0612
   -0.0351   -0.0593
   -0.0328   -0.0575
   -0.0306   -0.0557
   -0.0286   -0.0539
   -0.0266   -0.0522
   -0.0248   -0.0505
   -0.0230   -0.0489
   -0.0214   -0.0473
   -0.0198   -0.0457
   -0.0183   -0.0442
   -0.0169   -0.0427
   -0.0156   -0.0413
   -0.0144   -0.0399
   -0.0132   -0.0385
   -0.0121   -0.0372
   -0.0110   -0.0359
   -0.0101   -0.0346
   -0.0091   -0.0334
   -0.0083   -0.0322
   -0.0074   -0.0310
   -0.0067   -0.0299
   -0.0060   -0.0288
   -0.0053   -0.0278
   -0.0047   -0.0267
   -0.0041   -0.0257
   -0.0035   -0.0248
   -0.0030   -0.0238
   -0.0025   -0.0229
   -0.0021   -0.0221
   -0.0017   -0.0212
   -0.0013   -0.0204
   -0.0009   -0.0196
   -0.0006   -0.0188
   -0.0003   -0.0181
    0.0000   -0.0174
    0.0003   -0.0181
    0.0006   -0.0188
    0.0009   -0.0196
    0.0013   -0.0204
    0.0017   -0.0212
    0.0021   -0.0221
    0.0025   -0.0229
    0.0030   -0.0238
    0.0035   -0.0248
    0.0041   -0.0257
    0.0047   -0.0267
    0.0053   -0.0278
    0.0060   -0.0288
    0.0067   -0.0299
    0.0074   -0.0310
    0.0083   -0.0322
    0.0091   -0.0334
    0.0101   -0.0346
    0.0110   -0.0359
    0.0121   -0.0372
    0.0132   -0.0385
    0.0144   -0.0399
    0.0156   -0.0413
    0.0169   -0.0427
    0.0183   -0.0442
    0.0198   -0.0457
    0.0214   -0.0473
    0.0230   -0.0489
    0.0248   -0.0505
    0.0266   -0.0522
    0.0286   -0.0539
    0.0306   -0.0557
    0.0328   -0.0575
    0.0351   -0.0593
    0.0375   -0.0612
    0.0400   -0.0631
    0.0427   -0.0651
    0.0456   -0.0670
    0.0485   -0.0691
    0.0517   -0.0711
    0.0550   -0.0732
    0.0584   -0.0753
    0.0621   -0.0775
    0.0659   -0.0796
    0.0699   -0.0819
    0.0741   -0.0841
    0.0786   -0.0863
    0.0832   -0.0886
    0.0881   -0.0909
    0.0932   -0.0932
    0.0986   -0.0955
    0.1042   -0.0979
    0.1101   -0.1002
    0.1163   -0.1025
    0.1228   -0.1048
    0.1295   -0.1072
    0.1366   -0.1095
    0.1440   -0.1117
    0.1518   -0.1140
    0.1599   -0.1162
    0.1684   -0.1184
    0.1773   -0.1205
    0.1866   -0.1226
    0.1963   -0.1246
    0.2064   -0.1265
    0.2170   -0.1283
    0.2280   -0.1301
    0.2396   -0.1317
    0.2516   -0.1332
    0.2642   -0.1346
    0.2773   -0.1358
    0.2909   -0.1369
    0.3051   -0.1378
    0.3200   -0.1385
    0.3354   -0.1389
    0.3515   -0.1392
    0.3683   -0.1392
    0.3858   -0.1389
    0.4039   -0.1383
    0.4229   -0.1374
    0.4425   -0.1361
    0.4630   -0.1345
    0.4843   -0.1325
    0.5064   -0.1300
    0.5294   -0.1271
    0.5534   -0.1237
    0.5782   -0.1197
    0.6040   -0.1152
    0.6308   -0.1101
    0.6586   -0.1043
    0.6875   -0.0978
    0.7174   -0.0906
    0.7485   -0.0826
    0.7807   -0.0738
    0.8141   -0.0641
    0.8487   -0.0534
    0.8845   -0.0417
    0.9217   -0.0290
    0.9602   -0.0151
    1.0000         0
    0.9602    0.0151
    0.9217    0.0290
    0.8845    0.0417
    0.8487    0.0534
    0.8141    0.0641
    0.7807    0.0738
    0.7485    0.0826
    0.7174    0.0906
    0.6875    0.0978
    0.6586    0.1043
    0.6308    0.1101
    0.6040    0.1152
    0.5782    0.1197
    0.5534    0.1237
    0.5294    0.1271
    0.5064    0.1300
    0.4843    0.1325
    0.4630    0.1345
    0.4425    0.1361
    0.4229    0.1374
    0.4039    0.1383
    0.3858    0.1389
    0.3683    0.1392
    0.3515    0.1392
    0.3354    0.1389
    0.3200    0.1385
    0.3051    0.1378
    0.2909    0.1369
    0.2773    0.1358
    0.2642    0.1346
    0.2516    0.1332
    0.2396    0.1317
    0.2280    0.1301
    0.2170    0.1283
    0.2064    0.1265
    0.1963    0.1246
    0.1866    0.1226
    0.1773    0.1205
    0.1684    0.1184
    0.1599    0.1162
    0.1518    0.1140
    0.1440    0.1117
    0.1366    0.1095
    0.1295    0.1072
    0.1228    0.1048
    0.1163    0.1025
    0.1101    0.1002
    0.1042    0.0979
    0.0986    0.0955
    0.0932    0.0932
    0.0881    0.0909
    0.0832    0.0886
    0.0786    0.0863
    0.0741    0.0841
    0.0699    0.0819
    0.0659    0.0796
    0.0621    0.0775
    0.0584    0.0753
    0.0550    0.0732
    0.0517    0.0711
    0.0485    0.0691
    0.0456    0.0670
    0.0427    0.0651
    0.0400    0.0631
    0.0375    0.0612
    0.0351    0.0593
    0.0328    0.0575
    0.0306    0.0557
    0.0286    0.0539
    0.0266    0.0522
    0.0248    0.0505
    0.0230    0.0489
    0.0214    0.0473
    0.0198    0.0457
    0.0183    0.0442
    0.0169    0.0427
    0.0156    0.0413
    0.0144    0.0399
    0.0132    0.0385
    0.0121    0.0372
    0.0110    0.0359
    0.0101    0.0346
    0.0091    0.0334
    0.0083    0.0322
    0.0074    0.0310
    0.0067    0.0299
    0.0060    0.0288
    0.0053    0.0278
    0.0047    0.0267
    0.0041    0.0257
    0.0035    0.0248
    0.0030    0.0238
    0.0025    0.0229
    0.0021    0.0221
    0.0017    0.0212
    0.0013    0.0204
    0.0009    0.0196
    0.0006    0.0188
    0.0003    0.0181
    0.0000    0.0174
   -0.0003    0.0181
   -0.0006    0.0188
   -0.0009    0.0196
   -0.0013    0.0204
   -0.0017    0.0212
   -0.0021    0.0221
   -0.0025    0.0229
   -0.0030    0.0238
   -0.0035    0.0248
   -0.0041    0.0257
   -0.0047    0.0267
   -0.0053    0.0278
   -0.0060    0.0288
   -0.0067    0.0299
   -0.0074    0.0310
   -0.0083    0.0322
   -0.0091    0.0334
   -0.0101    0.0346
   -0.0110    0.0359
   -0.0121    0.0372
   -0.0132    0.0385
   -0.0144    0.0399
   -0.0156    0.0413
   -0.0169    0.0427
   -0.0183    0.0442
   -0.0198    0.0457
   -0.0214    0.0473
   -0.0230    0.0489
   -0.0248    0.0505
   -0.0266    0.0522
   -0.0286    0.0539
   -0.0306    0.0557
   -0.0328    0.0575
   -0.0351    0.0593
   -0.0375    0.0612
   -0.0400    0.0631
   -0.0427    0.0651
   -0.0456    0.0670
   -0.0485    0.0691
   -0.0517    0.0711
   -0.0550    0.0732
   -0.0584    0.0753
   -0.0621    0.0775
   -0.0659    0.0796
   -0.0699    0.0819
   -0.0741    0.0841
   -0.0786    0.0863
   -0.0832    0.0886
   -0.0881    0.0909
   -0.0932    0.0932
   -0.0986    0.0955
   -0.1042    0.0979
   -0.1101    0.1002
   -0.1163    0.1025
   -0.1228    0.1048
   -0.1295    0.1072
   -0.1366    0.1095
   -0.1440    0.1117
   -0.1518    0.1140
   -0.1599    0.1162
   -0.1684    0.1184
   -0.1773    0.1205
   -0.1866    0.1226
   -0.1963    0.1246
   -0.2064    0.1265
   -0.2170    0.1283
   -0.2280    0.1301
   -0.2396    0.1317
   -0.2516    0.1332
   -0.2642    0.1346
   -0.2773    0.1358
   -0.2909    0.1369
   -0.3051    0.1378
   -0.3200    0.1385
   -0.3354    0.1389
   -0.3515    0.1392
   -0.3683    0.1392
   -0.3858    0.1389
   -0.4039    0.1383
   -0.4229    0.1374
   -0.4425    0.1361
   -0.4630    0.1345
   -0.4843    0.1325
   -0.5064    0.1300
   -0.5294    0.1271
   -0.5534    0.1237
   -0.5782    0.1197
   -0.6040    0.1152
   -0.6308    0.1101
   -0.6586    0.1043
   -0.6875    0.0978
   -0.7174    0.0906
   -0.7485    0.0826
   -0.7807    0.0738
   -0.8141    0.0641
   -0.8487    0.0534
   -0.8845    0.0417
   -0.9217    0.0290
   -0.9602    0.0151
   -1.0000    0.0000

